Hallucinations or Attention Misdirection? The Path to Strategic Value Extraction in Business Using Large Language Models

Large Language Models with transformer architecture have revolutionized the domain of text generation, setting unprecedented benchmarks. Despite their impressive capabilities, LLMs have been criticized for generating outcomes that deviate from factual accuracy or display logical inconsistencies, phenomena commonly referred to as hallucinations. This term, however, has often been misapplied to any results deviating from the instructor's expectations, which this paper defines as attention misdirection rather than true hallucinations. Understanding the distinction between hallucinations and attention misdirection becomes increasingly relevant in business contexts, where the ramifications of such errors can significantly impact the value extraction from these inherently pre-trained models. This paper highlights the best practices of the PGI, Persona, Grouping, and Intelligence, method, a strategic framework that achieved a remarkable error rate of only 3,15 percent across 4,000 responses generated by GPT in response to a real business challenge. It emphasizes that by equipping experimentation with knowledge, businesses can unlock opportunities for innovation through the use of these natively pre-trained models. This reinforces the notion that strategic application grounded in a skilled team can maximize the benefits of emergent technologies such as the LLMs.

==> jmlr_coverletter.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``\red{Manuscript Title}'' to the \emph{Journal of Machine Learning Research}.

Our manuscript studies \red{X, Y, and Z} which is important because of \red{A, B, and C}.

This paper extends our work of \red{Conference Paper} by addressing \red{X, Y, and Z additional points}.

We suggest the following action editors and referees for our submission.

Action Editors:
\begin{itemize}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
\end{itemize}

Reviewers:
\begin{itemize}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
\end{itemize}

Our submission has the following keywords: \red{keyword}, \red{keyword}, \red{keyword}, \red{keyword}, \red{keyword}.

As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

\red{Co-Author (Institution)}\\
\red{Co-Author (Institution)}\\
\red{Co-Author (Institution)}\\
\red{Co-Author (Institution)}

\end{document}







































